On gauge freedom, conservativity and intrinsic dimensionality estimation in diffusion models

Diffusion models are generative models that have recently demonstrated impressive performances in terms of sampling quality and density estimation in high dimensions. They rely on a forward continuous diffusion process and a backward continuous denoising process, which can be described by a time-dependent vector field and is used as a generative model. In the original formulation of the diffusion model, this vector field is assumed to be the score function (i.e. it is the gradient of the log-probability at a given time in the diffusion process). Curiously, on the practical side, most studies on diffusion models implement this vector field as a neural network function and do not constrain it be the gradient of some energy function (that is, most studies do not constrain the vector field to be conservative). Even though some studies investigated empirically whether such a constraint will lead to a performance gain, they lead to contradicting results and failed to provide analytical results. Here, we provide three analytical results regarding the extent of the modeling freedom of this vector field. {Firstly, we propose a novel decomposition of vector fields into a conservative component and an orthogonal component which satisfies a given (gauge) freedom. Secondly, from this orthogonal decomposition, we show that exact density estimation and exact sampling is achieved when the conservative component is exactly equals to the true score and therefore conservativity is neither necessary nor sufficient to obtain exact density estimation and exact sampling. Finally, we show that when it comes to inferring local information of the data manifold, constraining the vector field to be conservative is desirable.

==> bad_news.tex <==
\section{An exact density estimator can be a bad generator}\label{sec:good_density}
We show that for both a conservative and non-conservative vector field, the corresponding density estimator can be \textsl{exact} even though the model generates \textsl{bad} samples. We set the drift term $f(\mathbf{x},t)$ to be equal to $\mathbf{0}$ for simplicity.

\textbf{For non-conservative vector fields:}\\
Let  $s_{\theta}$ be a vector field which is very close to the true score $\nabla \log p_t(\mathbf{x})$. We assume that there exists a rotation field $R_t:\mathbb{R}^D \to \mathbb{R}^D$ with $\nabla \cdot R_t(\mathbf{x})=0$ such that
\begin{equation}\label{eq:helmholtz}
	s_{\theta}(\mathbf{x},t) = \nabla \log p_t(\mathbf{x}) + R_t(\mathbf{x}).
\end{equation}
Such a composing of a vector field into a conservative one and a rotation field is known as \textsl{Helmholtz decomposition} \cite{ton_tran_cong_helmholtzs_1993}. 
%If $R_t(\mathbf{x}) \neq 0$,  $s_{\theta}$ is not a conservative vector field. 
Using $s_{\theta}(\mathbf{x},t)$ to evaluate the model likelihood in equation (\ref{eq:density_estimation}) will lead to the exact likelihood because
\begin{align}\label{eq:trace}
	\rm{Tr} \left( \nabla s_{\theta}(\mathbf{x},t) \right) &= \rm{Tr} \left( \nabla^2 \log p_t(\mathbf{x}) \right) + \rm{Tr} (\nabla R_t(\mathbf{x}))  \notag \\
& =   \rm{Tr} \left( \nabla^2 \log p_t(\mathbf{x} \right) + \nabla \cdot R_t(\mathbf{x})   \notag \\
& =  \rm{Tr} \left(  \nabla^2 \log p_t(\mathbf{x}) \right)	
\end{align}
as the trace of the Jacobian of $R_t$ is equal to the divergence of $R_t$ which is $0$ by construction. Therefore, $s_{\theta}$ as defined in equation (\ref{eq:helmholtz}) yields an exact density estimator when using equation (\ref{eq:density_estimation}) to estimate $p_0(\mathbf{x}(0))$.

Moreover, the rotation field $R_t$ is expressing how close  $s_{\theta}$ is to the true score $ \log p_t(\mathbf{x})$. We may choose it freely as long it is the curl of a vector field $F$ on the one hand (since in that case $\nabla \cdot (\nabla \times F(\mathbf{x})) = 0$), and as long it is not a conservative vector field on the other hand.
%
%In particular, we can choose $R_t(\mathbf{x})$ independent of $x$ such that $||s_{\theta}(\mathbf{x},t) - \nabla \log p_t (\mathbf{x})||^2 = ||R_t(\mathbf{x})||^2 = \varepsilon^2 $ for an arbitrary $\varepsilon>0$. 

For example, consider $D=3$ and set $F_t(\mathbf{x}) = (0, 0.5\varepsilon x_1^2,0)^T$ which implies $R_t(\mathbf{x})=\nabla 
\times F_t(\mathbf{x}) =(0,0,\varepsilon x_1)^T$. Now if we use $s_{\theta}(\mathbf{x},t)$ for sampling, the initial value problem (\ref{eq:IVP_sampling}) turns into 
\begin{align}\label{eq:IVP_sampling_non-conservative}
	\begin{cases}
		d\bar{\mathbf{x}}(t) &= -\frac{1}{2}g(t)^2 \left[   \nabla \log p_t(\mathbf{x}) + \varepsilon x_1  \hat{e}_z \right] \\
		\bar{\mathbf{x}}(0)  &= \bar{\mathbf{x}}_0   
	\end{cases}
\end{align}
where $\hat{e}_z$ denotes the unit vector in $z-$direction. This vector field consists of a sum of two seperate vectors fields. Thus, the sum of the solutions to the seperate IVPs is a solution to the IVP (\ref{eq:IVP_sampling_non-conservative}) whenever the seperate initial values sum to $\bar{\mathbf{x}}_0$. However, the first term corresponds to the true data-generating ODE and thus will always lead to a sample $\mathbf{x}^*$ on the data-manifold whatever initial condition we choose. Therefore, a sample using $s_{\theta}$ from equation (\ref{eq:helmholtz}) can be written without loss of generality as
\begin{align}\label{eq:sample_non-conservative}
\mathbf{x} = \mathbf{x}^* - \frac{1}{2}\varepsilon z_0 \left( \int_{0}^{1} g(t)^2 x_1(t) \rm{dt} \right) \hat{e}_z
\end{align}
where $z_0 \neq 0$ is some real number. The integral in the bracket can be bounded from below as $g(t)$ is typically monotonically increasing, and a continuous function $x_1(t)$ attains its minimum in $[0,1]$. Thus,
\begin{align}\label{eq:sample1_lower_bound}
	||\mathbf{x}- \mathbf{x}^*||_2^2 =&  \left(\frac{1}{2}\varepsilon z_0  \int_{0}^{1} g(t)^2 x_1(t) \rm{dt} \right)^2 \notag \\
	\geq &   \left(\frac{1}{2}\varepsilon z_0  g(0)^2 \underset{t\in [0,1]}{\rm{min}}x_1(t) \right)^2.
\end{align}
A typical choice for $g(t)$ in practice is $g(t)=25^t$. Setting $\varepsilon = \frac{2}{z_0}$, we have that
\begin{align}\label{eq:sample1}
	||\mathbf{x}- \mathbf{x}^*||_2^2 \geq &   \left( \underset{t\in [0,1]}{\rm{min}}x_1(t) \right)^2.
\end{align}
Therefore, a sample generated by $s_{\theta}$  from equation (\ref{eq:helmholtz}) can deviate greatly from a true sample if the data-manifold is far away from the origin. Even if we preprocess the data to take values only in $[-1,1]$ we have that $	||\mathbf{x}- \mathbf{x}^*||_2^2 \geq 1$. It is straightforward to generalize this example to higher-dimensions than $3$.
% Recall that $g(t)^2$ is the diffusion coefficient and can in principal be choosen arbitrarily. For instance, \cite{song_score-based_2021} used for some experiments $g(t)= c \sigma^t$ with $c=1$ and $\sigma=25$. However, $c>0$ can in principle  be choosen arbitrary. Therefore, fixing $\varepsilon$ and setting $g(t) = \sigma^t / \sqrt{\varepsilon}$ implies that our sample obtained from $s_{\theta}(\mathbf{x},t)$ is given by 
%\begin{align}\label{eq:sample2}
%	\mathbf{x} = \mathbf{x}^* - \frac{1}{2} \frac{\sigma -1}{\log \sigma} \hat{e}_z
%\end{align}
%which can deviate greatly from $ \mathbf{x}^*$ for a large choice of $\sigma$, in particular, if the true density is concentrated in the $(x,y)-$plane.

Therefore, we have shown that even if a non-conservative  vector field $\{s_{\theta}(\mathbf{x},t)\}_{0\leq t \leq 1}$ yields the exact likelihood,
%\begin{enumerate}[label=\arabic*.] %roman, alph
%	\item $s_{\theta}(\mathbf{x},t)$ is $\varepsilon$-close to the true data generating distribution $\log p_t(\mathbf{x})$, that is $||s_{\theta}(\mathbf{x},t) - \log p_t(\mathbf{x})||^2 = \varepsilon^2$ for all $t\in [0,1]$, and
%	\item 
%\end{enumerate}
a sample generated by $\{s_{\theta}(\mathbf{x},t)\}_{0\leq t \leq 1}$ can be far from the sample generated by the true score $\{\nabla \log p_t (\mathbf{x})\}_{0\leq t \leq 1}$ .
%given by the training procedure described in Section \ref{sec:background}.  We assume that 

%\begin{remark}
%	Composing a vector field into a conservative one and a rotation field as in equation \ref{eq:helmholtz} is known \textsl{Helmholtz decomposition} \cite{ton_tran_cong_helmholtzs_1993} 
%\end{remark}

\textbf{For conservative vector fields:}\\
Let  $s_{\theta}$ be a conservative vector field of the form
\begin{equation}\label{eq:conservative_VF}
	s_{\theta}(\mathbf{x},t) = \nabla \log p_t(\mathbf{x}) + r(t) \boldsymbol{\varepsilon}.
\end{equation}
where $r(t):[0,\infty) \to \mathbb{R}$ and $\boldsymbol{\varepsilon} \in \mathbb{R}^D$ fixed. Note that $s_{\theta}(\mathbf{x},t)$ is conservative as it is the gradient of
\begin{equation}\label{eq:potential}
	\log p_t(\mathbf{x}) + r(t) \sum_{i=1}^{D} \varepsilon_i x_i .
\end{equation}

 That is, $s_{\theta}(\mathbf{x},t)$ is a noisy estimator of $ \nabla \log p_t(\mathbf{x}) $ with $r(t)$ and $\boldsymbol{\varepsilon}$ determining its deviation from the true score,
\begin{equation}\label{eq:distance_conservative}
	||s_{\theta}(\mathbf{x},t)- \nabla \log p_t(\mathbf{x})||^2 =  r(t)^2 || \mathbf{\varepsilon} ||^2.
\end{equation}
Since the second term of equation (\ref{eq:conservative_VF}) does not depend on $x$, we have that
\begin{align}\label{eq:trace_conservative}
	\rm{Tr} \left( \nabla s_{\theta}(\mathbf{x},t) \right) &= \rm{Tr} \left( \nabla^2 \log p_t(\mathbf{x}) \right) 
\end{align}
and therefore $s_\theta(\mathbf{x},t)$ yields exact densities when using equation (\ref{eq:density_estimation}) to estimate $p_0(\mathbf{x}(0))$.


The initial value problem (IVP) for sampling, equation (\ref{eq:IVP_sampling}), when using $s_\theta$ from equation (\ref{eq:conservative_VF}), is given by
\begin{align}\label{eq:IVP_sampling_conservative00}
	\begin{cases}
		d\bar{\mathbf{x}}(t) &= -\frac{1}{2}g(t)^2 \left[   \nabla \log p_t(\mathbf{x}) + r(t)\boldsymbol{\varepsilon} \right] \\
		\bar{\mathbf{x}}(0)  &= \bar{\mathbf{x}}_0   
	\end{cases}
\end{align}
This vector field consists of a sum of two seperate vectors fields - the first one depending on $\mathbf{x}$, and the second one independent of it. Therefore the two seperate vector fields commute and the solution of the IVP (\ref{eq:IVP_sampling_conservative00}) is given by the composition of the individual solutions. 

Thus, the sum of the solutions to the seperate IVPs is a solution to the IVP (\ref{eq:IVP_sampling_conservative00}) whenever the seperate initial values sum to $\bar{\mathbf{x}}_0$. As the solution to the second vector field is given by
\begin{align}\label{eq:solution_second}
	\mathbf{x}(t) =-\frac{1}{2}  \int_{0}^{t} g(s)^2 r(s)ds  \cdot \boldsymbol{\varepsilon}
\end{align}
the corresponding initial value is $0$. Therefore, a sample obtained from the IVP (\ref{eq:IVP_sampling_conservative00}) is given by
\begin{align}\label{eq:sample_conservative}
	\mathbf{x} = \mathbf{x}^* - \frac{1}{2}  \int_{0}^{1} g(t)^2 r(t) \rm{dt} \cdot \boldsymbol{\varepsilon}
\end{align}
where $ \mathbf{x}^*$ is a true sample from the data-generating distribution $p_0$.
Hence, depending on $g(t)$, $r(t)$ and $\boldsymbol{\varepsilon}$, a sample using the vector field (\ref{eq:conservative_VF}) can deviate greatly from $\mathbf{x}^*$ as
%especially in high-dimensions. For example, set $r(t)=2 g(t)^{-2}$, then 
\begin{align}\label{eq:distance_conservative}
||\mathbf{x} - \mathbf{x}^*||_2^2= \left(\frac{1}{2}  \int_{0}^{1} g(t)^2 r(t) \rm{dt}\right)^2 || \boldsymbol{\varepsilon}||_2^2.
\end{align}
For example, using $g(t)=25^t$, as it is done in some experiments in \cite{song_score-based_2021}, $r(t)=1$, we have
\begin{align}\label{eq:distance_conservative}
	||\mathbf{x} - \mathbf{x}^*||_2^2 \approx 2349 \cdot || \boldsymbol{\varepsilon}||_2^2.
\end{align}
for an arbitrary $ \boldsymbol{\varepsilon} \in \mathbb{R}^D$.
%where $\boldsymbol{\varepsilon} \sim \mathcal{N}(0,I)$.

Therefore, we have shown that even if a conservative  vector field $\{s_{\theta}(\mathbf{x},t)\}_{0\leq t \leq 1}$ yields the exact likelihood, a sample generated by $\{s_{\theta}(\mathbf{x},t)\}_{0\leq t \leq 1}$can be, in principle, arbitrarily far from the sample generated by the true score  $\{\nabla \log p_t (\mathbf{x})\}_{0\leq t \leq 1}$ .


==> data_generation.tex <==
\section{Conservativity is not necessary  for good data generation}\label{sec:good_generator}
We show that for both a conservative and non-conservative vector field, the model can generate \textsl{perfect} samples. 

First, we revisit some essential concepts from the theory of ordinary differential equations.  Let the initial value problem (IVP),
\begin{align}\label{eq:IVP_sampling}
	\begin{cases}
		d\bar{\mathbf{x}}_t &= u(\bar{\mathbf{x}}_t,t)dt \\
		\bar{\mathbf{x}}_0  &= \bar{\mathbf{x}}_0,
	\end{cases}
\end{align}
have the flow $\Phi^{u}_t(\bar{\mathbf{x}}_0)$ as its solution where we assume that $u$ is a complete vector field (see remark (\ref{rem:complete})). Similarily, let $\Phi^{v}_t(\bar{\mathbf{x}}_0)$ be the solution of the IVP (\ref{eq:IVP_sampling}) where we simply replace $u$ by $v$ (also complete). Then, a standard result in the theory of ordinary differential equations is that the solution to the IVP
\begin{align}\label{eq:IVP_good}
	\begin{cases}
		d\bar{\mathbf{x}}_t &= \left(u(\bar{\mathbf{x}}_t,t) + v(\bar{\mathbf{x}}_t,t)\right)dt \\
		\bar{\mathbf{x}}_0  &= \bar{\mathbf{x}}_0,
	\end{cases}
\end{align}
is given by $\Phi^{u+v}_t(\bar{\mathbf{x}}_0)= \left( \Phi^{u}_t \circ \Phi^{v}_t \right)(\bar{\mathbf{x}}_0)$ if and only if the two vector fields $h$ and $s$ commute, that is, if and only if  their Lie-bracket vanishes, $[u,v]=0$.

Now, let  $s_{\theta}$ be a vector field of the form
\begin{equation}\label{eq:helmholtz3}
	s_{\theta}(\mathbf{x},t) = \nabla \log p_t(\mathbf{x}) + r_t(\mathbf{x}).
\end{equation}
A sample  from  $s_{\theta}(\mathbf{x},t)$ is obtained by solving the following IVP 
\begin{align}\label{eq:IVP_sampling_conservative}
	\begin{cases}
		d\bar{\mathbf{x}}_t &=f(\mathbf{x}_t,t) -\frac{1}{2}g(t)^2 \left[   \nabla \log p_t(\mathbf{x}) + r_t(\mathbf{x}) \right], \\
		\bar{\mathbf{x}}_0 &= \bar{\mathbf{x}}_0.
	\end{cases}
\end{align}
which is the sum of two fector fields $u(\mathbf{x},t) := f(\mathbf{x}_t,t)  -\frac12 g(t)^2 \nabla \log p_t(\mathbf{x})$ and $v(\mathbf{x},t) := -\frac12 g(t)^2 r_t(\mathbf{x})$. Therefore, if $u$ and $v$ commute, that is $[u,v]=0$, we have that the solution to the IVP (\ref{eq:IVP_sampling_conservative}) is given by $\Phi^{u+v}_t(\bar{\mathbf{x}}_0)= \left( \Phi^{u}_t \circ \Phi^{v}_t \right)(\bar{\mathbf{x}}_0)$. Note that $\Phi^{u}_t$ is the flow of the true vector field and will thus generate a sample from the data generating distribution $p_0$ for all possible initial values. Hence, a sample generated by $\Phi^{u+v}_t$ will necessarily be a sample generated by $\Phi^{u}_t$, and therefore a sample from the data generating distribution $p_0$. 

How restrictive  is the condition $[u,v]=0$ on the remainder term $r_t(\mathbf{x})$? Since the Lie-bracket is linear, we have that  $[u,v]=0$ if and only if
\begin{align}\label{eq:}
&1.&   [f_t,r_t]&=0    \notag \\
&2.&    [\nabla \log p_t,r_t]&=0	
\end{align}
Note that typically, the drift term is given by $f(\mathbf{x},t)=\beta_t \mathbf{x}$ where $\{ \beta_t \}_{t\in [0,1]}$ is monotonicall increasing \cite{de_bortoli_convergence_2022}. Therefore, for all linear remainder terms, $r_t(\mathbf{x}) = A_t \mathbf{x}$, where $A_t$ is a time-dependent matrix, we have that 1. is always fullfilled as
\begin{align}\label{eq:}
	[f_t,r_t]& = \beta_t A_t \mathbf{x} - \beta_t A_t \mathbf{x} = \mathbf{0}.
\end{align}
Note that $r_t(\mathbf{x})$ is only conservative if $A_t$ is symmetric. Thus, condition 1. does not require conservativity of $s_{\theta}(\mathbf{x},t)$.

For 2. we additionally assume that $\nabla \log p_t(\mathbf{x})$ is Gaussian, that is $\nabla \log p_t (\mathbf{x}) = \Sigma_t \mathbf{x}$ and $\nabla^2 \log p_t (\mathbf{x}) = \Sigma_t$ for some time-dependent covariance function $ \Sigma_t$. Then, for condition 2., we have 
\begin{align}\label{eq:}
	[\nabla \log p_t,r_t]& =  A_t \Sigma_t \mathbf{x} -   \Sigma_t  A_t \mathbf{x} = \mathbf{0} \iff A_t \Sigma_t  =\Sigma_t  A_t 
\end{align}
Thus, $A_t$ and $\Sigma_t$ must commute.  For that, $A_t$ and $\Sigma_t$ need to be simultaneously diagonalizable which does not require for $A_t$ to be symmetric. Thus, also  condition 2. does not require conservativity of $s_{\theta}(\mathbf{x},t)$.

%of $r_t$ and therefore $s_{\theta}(\mathbf{x},t)$ as well.
%
%for a time dependent matrix $A_t$.
%If the drift term vanishes, that is $f(\mathbf{x},t)=\mathbf{0}$, the condition on $r_t$ is to commute of the true score $\nabla \log p_t$.


\begin{remark}\label{rem:complete}
The above derivations requires $h$ and $s$ to be complete vector fields. For example, any smooth vector field on a compact manifold is complete. In general, $u(\mathbf{x},t) := -\frac12 g(t)^2 \nabla \log p_t(\mathbf{x})$  must not be complete as its support is not necessarily compact. However, also the instantenous change of variable formula used to estimate the density, see equation (\ref{eq:density_estimation}), requires $\mathbf{x}(t)$  to be a finite random variable for all $t$, see theorem 1 in \cite{chen_neural_2018}. Even though this is not true since the increments of $\mathbf{x}(t)$ are Gaussian, it  is practically fulfilled since the variance of that Gaussian is infinitesimal small. Similarly, we can assume that practically $u(\mathbf{x},t)$ is complete.
%Nevertheless, equation (\ref{eq:density_estimation}) is commonly used to estimate the density
\end{remark}




==> data_generation2.tex <==
\section{Conservativity is not necessary  for good data generation}\label{sec:good_generator}
We show that also for a non-conservative vector field, the model can generate \textsl{exact} samples. 
%We derive the result for the typical use-case of diffusion models where the drift and diffusion coefficients, $f$ and $g$, are given by $f(\mathbf{x},t)=-\frac12 \beta(t) \mathbf{x}$ and $g(t)= \sqrt{\beta(t)}$, respectively.  Note that $t\mapsto \beta(t)$ is a positive, monotonically increasing scalar function to ensure convergence of the forward SDE to a standard Gaussian  \cite{song_score-based_2021,de_bortoli_convergence_2022,nichol_improved_2021}. For the general case, we refer to the supplementary material.

%First, we revisit some essential concepts from the theory of ordinary differential equations (ODEs), in particular, the concept of commuting vector fields. 
Our idea is based on the following standard result in the theory of ordinary differential equations (ODEs): the solution of a sum of two commuting vector fields is given by the compositions of their flows. Thus, if one of the flows is guaranteed to produce a sample on the manifold for any initial condition, their sum will also produce a sample on the manifold. 

 Concretely, let $s_{\theta}$ be defined by
\begin{equation}\label{eq:helmholtz3}
	s_{\theta}(\mathbf{x},t) = \nabla \log p_{t}(\mathbf{x}) + r_{t}(\mathbf{x}).
\end{equation}
Using $s_{\theta}$ for sampling, the ODE (\ref{eq:IVP_sampling}) can be written as
\begin{align}\label{eq:IVP_good}
	\begin{cases}
		d\mathbf{x}_{\tau} & = \left[ u(\mathbf{x}_{\tau},\tau) +v(\mathbf{x}_{\tau},\tau) \right] d\tau \\
		\mathbf{x}_0  &= \mathbf{x}_{\rm{init}},
	\end{cases}
\end{align}
where $u(\mathbf{x}_{\tau},\tau) =- f(\mathbf{x}_{\tau},\tau) + \frac12 g^2(\tau)\nabla \log p_{\tau}(\mathbf{x}_{\tau})$ and $v(\mathbf{x}_{\tau},\tau) = \frac12 g^2(\tau) r_{\tau}(\mathbf{x}_{\tau})$. Let $\phi_{\tau}^u$ denote the flow of the vector field $u(\mathbf{x}_{\tau},\tau)$, that is the solution to the IVP (\ref{eq:IVP_good}) with $v=\mathbf{0}$.
The flow $\phi_{1}^u$ always generates a sample on the manifold as it corresponds to the true vector field from equation (\ref{eq:backward_equation}).  

When does $\phi_{\tau}^u$ commutes with $\phi_{\tau}^v$? If $u$ and $v$ do not explicitely depend on $\tau$, that is $u(\mathbf{x}_{\tau},\tau) = u(\mathbf{x}_{\tau})$ and $v(\mathbf{x}_{\tau},\tau) = v(\mathbf{x}_{\tau})$, we have that the flow of the sum of $u$ and $v$ is given by the composition of $\phi_{\tau}^u$ and $\phi_{\tau}^v$ whenever the Lie-bracket $[u,v]$ vanishes, that is whenever $[u,v]=0$. We generalize this result for the sum of time-dependent vector fields in the following. For that, we lift up the state variable $\mathbf{x}_{\tau}$ by one dimension by defining $\breve{\mathbf{x}}=(\mathbf{x},\tau)$. Then, the IVP (\ref{eq:IVP_good}) turns into 
\begin{align}\label{eq:IVP_lifted}
	\begin{cases}
		d\breve{\mathbf{x}}_{\tau} & = \left[ U(\breve{\mathbf{x}}) +V(\breve{\mathbf{x}}) \right] d\tau \\
		\breve{\mathbf{x}}_0  &= \breve{\mathbf{x}}_{\rm{init}},
	\end{cases}
\end{align}
where $U(\breve{\mathbf{x}}) = (u(\mathbf{x}_{\tau},\tau),\alpha)$ and $V(\breve{\mathbf{x}}) = (v(\mathbf{x}_{\tau},\tau),\beta)$ where $\alpha,\beta \in \mathbb{R}$ such that $\alpha + \beta = 1$. The vector fields $U$ and $V$ do not explicitely depend on $\tau$ and thus the flow of the IVP (\ref{eq:IVP_lifted}) is given by the composition of the flows $\phi_{\tau}^{U}$ and $\phi_{\tau}^{U}$ whenever their Lie-bracket vanishes,
\begin{align}\label{eq:commuting_VF}
	&\quad &  [U,V] =& \mathbf{0}    \notag \\
	&\iff & \nabla_{(\mathbf{x},\tau)} V U - \nabla_{(\mathbf{x},\tau)} U V  =& \mathbf{0}  \notag \\
	&\iff & \alpha \frac{\partial v(\mathbf{x}_{\tau},\tau)} {\tau} - \beta \frac{\partial u(\mathbf{x}_{\tau},\tau)}{\tau}  + \nabla_{\mathbf{x}} v(\mathbf{x}_{\tau},\tau) u(\mathbf{x}_{\tau},\tau) - \nabla_{\mathbf{x}} u(\mathbf{x}_{\tau},\tau) v(\mathbf{x}_{\tau},\tau) =& \mathbf{0} \notag \\
	&\iff & \alpha \frac{\partial v(\mathbf{x}_{\tau},\tau)} {\tau} - \beta \frac{\partial u(\mathbf{x}_{\tau},\tau)}{\tau}  + [u(\mathbf{x}_{\tau},\tau),v(\mathbf{x}_{\tau},\tau)] =& \mathbf{0} \notag \\
		&\iff &[u,v]   =&   \frac{\partial \left( \beta u-\alpha v \right) } {\tau} 
                       \end{align}
where in the last step we have skipped the dependencies on $(\mathbf{x}_{\tau},\tau)$ for convenience. Therefore, whenever $\frac{\partial \left( \beta u- \alpha v \right) } {\tau}  = [u,v] $ for all $\tau \in [0,1]$, we have that 
\begin{equation}
	\phi^{U+V}_{\tau} (\breve{\mathbf{x}}_{\rm{init}}) =  \left( \phi^{U}_{\tau} \circ \phi^{V}_{\tau}  \right) (\breve{\mathbf{x}}_{\rm{init}}) 
\end{equation}
where $ \phi^{U}_{\tau}(\breve{\mathbf{x}}_{\rm{init}})  = ( \phi^{u}_{\tau}(\mathbf{x}_{\rm{init}}) , \alpha \tau + \tau_{\rm{init}}) $ and  $\phi^{V}_{\tau}(\breve{\mathbf{x}}_{\rm{init}})   = ( \phi^{v}_{\tau}(\mathbf{x}_{\rm{init}}), \beta \tau + \tau_{\rm{init}} )$.
 As $\phi_1^u$ generates a sample on the manifold for any initial condition, a sample generated by the IVP (\ref{eq:IVP_lifted}) at time $\tau=1$ is given by $(\mathbf{x}^*,1)$. A solution to the IVP (\ref{eq:IVP_good}), which is the projection of the solution of the IVP (\ref{eq:IVP_lifted}) onto the first $D$ dimensions, thus always provides a sample on the manifold.
 
 What remains to show is that $\frac{\partial \left( \beta u- \alpha v \right) } {\tau}  = [v,u] $ is possible for a conservative vector field $u$ and a non-conservative vector field $v$. It is sufficient to construct a non-trivial counterexample. For that, we set $ \alpha v = \beta u  + \psi$ where $\psi$ is time-independent. Then, condition (\ref{eq:commuting_VF}) turns into
 \begin{align}\label{eq:commuting_countererExp}
 &\quad& [u,v]   =&   \frac{\partial \left( \beta u-\alpha v \right) } {\tau}    \notag \\
 &\iff & [u,\beta u + \psi ] =& \frac{\partial \psi  } {\tau}   \notag \\
 &\iff & \beta  [u,u] + [u, \psi ] =& \frac{\partial \psi  } {\tau}    \notag \\
  &\iff &  [u, \psi ] =& \mathbf{0}.  \notag \\
 \end{align}
Hence, it is enough to show that  $[u, \psi ] =0$ is possible for a conservative $u$ and a non-conservative $\psi$. Remember that $u(\mathbf{x}_{\tau},\tau) =- f(\mathbf{x}_{\tau},\tau) + \frac12 g^2(\tau)\nabla \log p_{\tau}(\mathbf{x}_{\tau})$. Typically in diffusion models, $f(\mathbf{x},\tau)=-\frac12 \beta(\tau) \mathbf{x}$ and $g(t)= \sqrt{\beta(\tau)}$, respectively, where  $\tau\mapsto \beta(\tau)$ is a positive, monotonically increasing scalar function to ensure convergence of the forward SDE to a standard Gaussian  \cite{song_score-based_2021,de_bortoli_convergence_2022,nichol_improved_2021}. With that choice, we have that $\nabla_{\mathbf{x}} u(\mathbf{x}_{\tau},\tau) = \frac12 \beta(\tau) I +\frac12 \beta(\tau) \nabla^2_{\mathbf{x}} \log p_{\tau}(\mathbf{x}_{\tau})$ and thus condition (\ref{eq:commuting_countererExp}) turns into 
 \begin{align}\label{eq:commuting_countererExp2}
	&\quad& [u, \psi ]  = \mathbf{0}&      \notag \\
	&\iff & [- f(\mathbf{x}_{\tau},\tau) + \frac12 g^2(\tau)\nabla \log p_{\tau}(\mathbf{x}_{\tau}), \psi ] =& \mathbf{0}  \notag \\
	&\iff &  [- f(\mathbf{x}_{\tau},\tau) ,\psi] + \frac12 g^2(\tau) [ \nabla_{\mathbf{x}} \log p_{\tau}(\mathbf{x}_{\tau}), \psi ] =& \mathbf{0}  \notag \\
	&\iff &  \beta(\tau)[ \mathbf{x},\psi] + \frac12 \beta(\tau) [ \nabla_{\mathbf{x}} \log p_{\tau}(\mathbf{x}_{\tau}), \psi ] =& \mathbf{0}  \notag \\
	\end{align}
Next we assume that $\psi$ is linear, that is $\psi (\mathbf{x}) = A \mathbf{x}$ for some time-independent matrix $A$. Then, $[ \mathbf{x},\psi ] =\mathbf{0}$ and what remains to show is that
\begin{equation}\label{eq:commuting_final}
[ \nabla_{\mathbf{x}} \log p_{\tau}(\mathbf{x}_{\tau}),  A \mathbf{x} ] = \mathbf{0}.
\end{equation}
Finally, we assume that $\log p_{\tau}(\mathbf{x}_{\tau})$ is Gaussian such that $\nabla_{\mathbf{x}} \log p_{\tau}(\mathbf{x}_{\tau}) = \Sigma_{\tau} \mathbf{x}$. Condition (\ref{eq:commuting_final}) is then equivalent to the Lie-bracket of $\Sigma_t$ and $A$ to vanish, that is $[\Sigma_{\tau},A] =\mathbf{0}$. The latter is possible for all $\tau$ even though $A$ is not symmetric. For example, consider 
\begin{equation}
	\Sigma_t = \left( \begin{matrix}
		\sigma_1(t) & 0 & 0\\
		0 & \sigma_1(t) & 0 \\
		0 & 0 & \sigma_2(t)
	\end{matrix} \right) \qquad \text{and} \qquad A = \left( \begin{matrix}
		a & b & 0\\
		c & d & 0 \\
		0 & 0 & e
	\end{matrix} \right)  
\end{equation}
where $\sigma_1(t),\sigma_2(t)>0$, and  $a,b,c,d,e \in \mathbb{R}$.  Whenever $b\neq c$, the matrix $A$ is not symmetric and thus $\psi$ is not conservative. Thus, we have constructed a non-trivial counter example (which can be straightforwardly generalized to arbitrary high-dimensions) showing that conservativity is not necessary for generating an exact sample on the manifold.

\begin{remark}
	There is a degree of freedom on how to lift   ODE (\ref{eq:IVP_good}) to ODE (\ref{eq:IVP_lifted}) expressed in terms of the constraint $\alpha+\beta = 1$.  We have shown that conservativity is not necessary almost surely (namely whenever  $\alpha \neq 0$). However, if $\alpha=0$, we end up with the interesting condition that $[u,v]=\frac{\partial u}{\partial \tau}$ which is generally difficult to solve for $u$. 
%	Therefore, the result that conservativity is not necessary is only true in an almost sure sense. 
\end{remark}

==> exact_density.tex <==
\section{Conservativity is not necessary for good density estimation}\label{sec:good_density}
We show that for both a conservative and non-conservative vector field, the corresponding density estimator can be \textsl{exact}. For this section, we assume without any loss of generality that the forward SDE, equation (\ref{eq:forward_equation}), has no drift term, that is $f(\mathbf{x}_t,t)=\mathbf{0}$.

Let  $s_{\theta}$ be a vector field that is close to the true score $\nabla \log p_t(\mathbf{x})$. We assume that there exists a rotation field $R_t:\mathbb{R}^D \to \mathbb{R}^D$ with $\nabla \cdot R_t(\mathbf{x})=0$ such that
\begin{equation}\label{eq:helmholtz}
	s_{\theta}(\mathbf{x},t) = \nabla \log p_t(\mathbf{x}) + R_t(\mathbf{x}).
\end{equation}
Such a composition of a vector field into a conservative one and a rotation field is known as \textsl{Helmholtz decomposition} in physics \cite{ton_tran_cong_helmholtzs_1993}. For example, for every vector field which decays faster than $||\mathbf{x}||_2^{-n}$ for $||\mathbf{x}||_2 \to \infty$, $n>2$, such a decompisition exists \cite{glotzl_helmholtz_2023}.


Replacing the true score by $s_{\theta}(\mathbf{x},t)$ for evaluating the model likelihood in equation (\ref{eq:density_estimation}), will lead to the exact likelihood because
\begin{align}\label{eq:trace}
	{\rm{Tr}} \left( \nabla s_{\theta}(\mathbf{x},t) \right) &= {\rm{Tr}} \left( \nabla^2 \log p_t(\mathbf{x}) \right) + {\rm{Tr}} (\nabla R_t(\mathbf{x}))  \notag \\
	& =  { \rm{Tr} }\left( \nabla^2 \log p_t(\mathbf{x} \right) + \nabla \cdot R_t(\mathbf{x})   \notag \\
	& =  {\rm{Tr}} \left(  \nabla^2 \log p_t(\mathbf{x}) \right)	
\end{align}
as the trace of the Jacobian of $R_t$ is equal to the divergence of $R_t$ which is $0$ by construction. Therefore, $s_{\theta}$ as defined in equation (\ref{eq:helmholtz}) yields an exact density estimator when using equation (\ref{eq:density_estimation}) to estimate $p_0(\mathbf{x}_0)$, no matter how close $s_{\theta}$ is to the true score. 

Note that a rotation field is generally not conservative and therefore the vector field (\ref{eq:helmholtz}) is not conservative in general. However, if $R_t$ is independent of $\mathbf{x}$, the vector field (\ref{eq:helmholtz}) is conservative, and we still have that $\nabla \cdot R_t(\mathbf{x})= 0$. Therefore, we have shown that whenever $s_{\theta}$  is Helmholtz decomposable, the corresponding density estimator can be exact - independent of whether it is conservative or not. It will be exact when the conservative part matches to the true score. 

==> related_work.tex <==
\section{Related work}

Salisman and HO: 
- no difference in performance
- restircted archtiectures to be simialar for better comparison


Despite these findings, it is mathematically unsatisfactory to learn $s_{\theta}$ knowing that it is generally not consistent. This mathematical ghost is haunting the diffusion community which is reflected in a surge of recent papers addressing this conflict \cite{chao_investigating_2023,lai_improving_2023, wenliang_score-based_nodate, du_reduce_2023}. 

Why are they motivating to learn conservative VFs?

